Bunched Fuzz: Sensitivity for Vector Metrics

Program sensitivity measures the distance between the outputs of a program when run on two related inputs. This notion, which plays a key role in areas such as data privacy and optimization, has been the focus of several program analysis techniques introduced in recent years. Among the most successful ones, we can highlight type systems inspired by linear logic, as pioneered by Reed and Pierce in the Fuzz programming language. In Fuzz, each type is equipped with its own distance, and sensitivity analysis boils down to type checking. In particular, Fuzz features two product types, corresponding to two different notions of distance: the tensor product combines the distances of each component by adding them, while the with product takes their maximum. In this work, we show that these products can be generalized to arbitrary $L^p$ distances, metrics that are often used in privacy and optimization. The original Fuzz products, tensor and with, correspond to the special cases $L^1$ and $L^\infty$. To ease the handling of such products, we extend the Fuzz type system with bunches -- as in the logic of bunched implications -- where the distances of different groups of variables can be combined using different $L^p$ distances. We show that our extension can be used to reason about quantitative properties of probabilistic programs.

==> sect_examples.tex <==
In this section, we will look at some examples of programs and primitives that
illustrate the use of different \lp metrics in \system{}.

\paragraph{Rotations}

\aaa{Can we say anything when we vary $\theta$?}

As a warm-up, let us consider how we can extend \system{} with a primitive for
computing rotations on the cartesian plane.  Given a rotation angle $\theta \in \R$, we
define the following function $R_\theta$:
\begin{align*}
  R_{\theta} & : \R^2 \to \R^2 \\
  R_\theta(x,y) & =(\cos(\theta)x- \sin(\theta)y,\sin(\theta)x+\cos(\theta)y).
\end{align*}
Using the $L^2$ distance we have, for any $(x,y), (x',y') \in \mathbb R^2 $:
$$ d_{2}( R_{\theta}(x,y), R_{\theta}(x',y'))=d_{2}( (x,y),
(x',y')).$$ So, as a function on $(\R^2, d_2)$, $R_{\theta}$ is non-expansive.
In other words, it has type $\R \otimes_2 \R \multimap \R \otimes_2 \R$.

Note that, by contrast, $R_{\theta}$ is not non-expansive for the $L^1$ or
$L^\infty$ distances.  For instance, suppose that $\theta = \pi / 4$, and let
$p = (\sqrt{2}/2,\sqrt{2}/2)$. Then
\begin{align*}
  R_\theta(0,0) & = (0,0) &
  R_\theta(1,0) & = p &
  R_\theta(p) & = (0,1).
\end{align*}
Thus,
$d_{1}(R_\theta(0,0),R_\theta(1,0)) = \sqrt{2}/2 + \sqrt{2}/2 = \sqrt{2}$,
which is strictly larger than $d_{1}((0,0),(1,0)) = 1$.  Similarly,
$d_{\infty}(R_\theta(0,0),R_\theta(p)) = \max(0,1) = 1$,
which is strictly larger than
$d_{\infty}((0,0),p) = \max(\sqrt{2}/2,\sqrt{2}/2) =
\sqrt{2}/2$.

\paragraph{Computing distances}

Suppose that the type $X$ denotes a metric space where the triangle inequality
holds.  Then we can incorporate its distance function in \system{} with the type
\[ X \otimes_1 X \multimap \R. \]
Indeed, let $x$, $x'$, $y$ and $y'$ be arbitrary elements of $X$.  Then
\begin{align*}
d_X(x,y) - d_X(x',y')
& \leq d_X(x,x') + d_X(x',y') + d_X(y',y) - d_X(x',y') \\
& = d_X(x,x') + d_X(y,y') \\
& = d_1((x,y),(x',y')).
\end{align*}
By symmetry, we also know that $d_X(x',y') - d_X(x,y) \leq d_1((x,y),(x',y'))$.
Combined, these two facts show
\begin{align*}
  d_{\R}(d_X(x,y), d_X(x',y'))
  & = |d_X(x,y) - d_X(x',y')| \\
  & \leq d_1((x,y),(x',y')),
\end{align*}
which proves that $d_X$ is indeed a non-expansive function.

\paragraph{Currying and Uncurrying}

The last two examples illustrate how product types with different metrics can be
manipulated with primitives in a Fuzz-like type system.  Even before \system{},
other languages had already noted that such alternative metrics could be useful.
For example, the Duet language~\cite{DBLP:journals/pacmpl/NearDASGWSZSSS19}
features primitive vector and matrix types under the $L^2$ distance, which are
required for the Gaussian mechanism, one of the basic building blocks of
differential privacy.

The main novelty of \system{} is the use of bunches to simplify the manipulation
of such product types component wise (e.g., by doing case analysis).
Accordingly, we'll now shift gears and consider how the bunched environments of
\system{} allow us to simplify the use of such types.  To start, let us
illustrate the use of higher-order functions by implementing combinators for
currying and uncurrying.  These functions are well-typed, provided that the
functions and tensors that appear in the types share the same indices:
\begin{align*}
  curry &: ((A\otimes_p B) \multimap_p C) \multimap (A\multimap_p B \multimap_p C)\\
  curry &\;f \; x \; y = f (x, y)\\
  uncurry &: (A\multimap_p B \multimap_p C) \multimap ((A\otimes_p B) \multimap_p C).\\
  uncurry &\;f \; z = \LetPairIn{x}{y}{z}{f\; x\; y}
\end{align*}
The reason why the indices have to be the same can be traced back to the
$\multimap\mathrm{E}$ rule (cf. \Cref{fig:BunchedFuzzTypingRules}), which uses
the $,_p$ connective to eliminate $\multimap_p$ (cf. \Cref{fig:curry-deriv} in
the Appendix for a detailed derivation).  If the indices do not agree, currying
is not possible; in other words, we cannot in general soundly curry a function
of type $A\otimes_p B \multimap_q C$ to obtain something of type
$A \multimap_p B \multimap_q C$.  However, if $q \leq p$, note that it would be
possible to soundly view $A \otimes_q B$ as a subtype of $A \otimes_p B$, thanks
to \Cref{prop:relationTensors}.  In this case, we could then convert from
$A \otimes_p B \multimap_q C$ to $A \otimes_q B \multimap_q C$ (note the
variance), and then curry to obtain a function of type
$A \multimap_q B \multimap_q C$.

\aaa{We should include an example demonstrating why this is not sound in
  general.}

% \paragraph{Relations between $\otimes_p$ types}

% \note{PB: I am not sure whether the following properties should be
%   included in Sect. 5 or in this Examples section}

% \begin{proposition}\label{prop:relationTensors}
% \begin{enumerate}
% \item The identity map on pairs from the metric space $A \otimes_1 B$ to   $A
%  \otimes_2B$ is non-expansive. In other words the identity map
%  belongs to $A \otimes_1 B \multimap A \otimes_2B$.
% \item  The identity map belongs to $ !_{\sqrt {2}}(A \otimes_2 B)
%   \multimap A \otimes_1B$.
% \item  More generally, for $p \leq q$ the identity map belongs to:
%   $$A \otimes_p B \multimap A \otimes_qB$$
% $$ !_{2^ {1/p-1/q}} (A \otimes_q B) \multimap A \otimes_pB $$
% \end{enumerate}
% \end{proposition}
% \begin{proof}
% Point 1 and the first statement of 3 follow from the fact that
% $d_q (x,y) \leq d_p(x,y)$, by Prop. \ref{prop:relations_dp} (\ref{prop:relations_dp1}).
% %$\ell^q(x,y) \leq \ell^p(x,y)$ for $p \leq q$ and $x, y \in \R^{+}$.

% Consider point 2. It follows from $$d_1((x,y), (x',y') ) \leq
% \sqrt{2} \;  d_2((x,y), (x',y') ), $$ by
% Prop. \ref{prop:relations_dp} (\ref{prop:relations_dp2}) in the
% case $n=2$.
% % First for  $x, y \in \R^{+}$ we have $xy
% % \leq x^2+y^2$. Thus
% % $$(x+y)^2=x^2+2xy+y^2 \leq 2(x^2+y^2)$$
% % $$(x+y) \leq \sqrt {2}  \sqrt {(x^2+y^2)}$$
% % $$ \ell^1(x,y)  \leq \sqrt{2} \ell^2(x,y)$$

% The second statement of point 3 can be derived
%  from Prop.  \ref{prop:relations_dp} ( \ref{prop:relations_dp1})
%  in the case $n=2$.
% % from Holder's
% % inequality:
% % $$\ell^p(x,y) \leq 2^{1/p-1/q}\ell^q(x,y)$$
% \end{proof}
% \begin{remark}\label{remark:tensorinclusions}
% Note that a consequence of point 1 of Prop. \ref{prop:relationTensors}
% is that if a function $f$ belongs to a space $A \otimes_2 B \multimap
% C$, then it also belongs to $A \otimes_1 B \multimap
% C$. We can thus write:
% $$ (A \otimes_2 B \multimap
% C)  \; \subseteq   \;  A \otimes_1 B \multimap
% C$$
% Similarly from point 2 we can deduce:
% $$ (A \otimes_1 B \multimap
% C) \; \subseteq   \;  (!_{\sqrt {2}} (A \otimes_2 B) \multimap
% C)$$
% Analogous inclusions can be derived from points 3 and 4.
% \end{remark}
% \pb{Should we say that a consequence of this remark is that we could add to our type
%   system some subtyping rules suggested by these inclusions, and that
%   the soundness of the interpretation in metrics spaces would be
%   preserved ?}

\paragraph{Precise sensitivity for functions with multiple arguments}

Another useful feature of \system{} is that its contraction rule allows us to
split sensitivities more accurately than if we used the contraction rule that is
derivable in the original Fuzz.  Concretely, suppose that we have a program of
the form $\lambda p. \LetPairIn{x}{y}{p} f(x,y) + g(x,y)$, where $f$ and $g$
have types
\begin{align*}
  &f : (!_2\R) \otimes_2 \R \multimap \R\\
  &g : \R \otimes_2 (!_2\R) \multimap \R,
\end{align*}
and where we have elided the wrapping and unwrapping of $!$ types, for
simplicity.

Let us sketch how this program is typed in \system{}. Addition belongs to
$\R \otimes_1 \R \multimap \R$, so by \Cref{prop:relationTensors} it can also be
given the type $!_{\sqrt {2}} (\R \otimes_2 \R) \multimap \R$. Thus, we can
build the following derivation for the body of the program:
\begin{mathpar}
  \inferrule*[Left=2Contr]{
\Gamma \vdash  f(x_1,y_1) + g(x_2,y_2) : \R }
 {[x :\R ]_{\sqrt {10}} \; ,_2 [y :\R ]_{\sqrt {10}} \vdash  f(x,y) + g(x,y) : \R }
\end{mathpar}
% \begin{mathpar}
%   \inferrule*[Left=2Contr]{
% [x_1 :\R ]_{2\sqrt {2}} ,_2 [y_1 :\R ]_{\sqrt {2}} ,_2 [x_2 :\R
% ]_{\sqrt {2}} ,_2 [y_2 :\R ]_{2\sqrt {2}} \vdash  f(x_1,y_1) + g(x_2,y_2) : \R }
%  {[x :\R ]_{\sqrt {10}} \; ,_2 [y :\R ]_{\sqrt {10}} \vdash  f(x,y) + g(x,y) : \R }
% \end{mathpar}
where
$\Gamma= ([x_1 :\R ]_{2\sqrt {2}} ,_2 [y_1 :\R ]_{\sqrt {2}}) ,_2 ([x_2 :\R
]_{\sqrt {2}} ,_2 [y_2 :\R ]_{2\sqrt {2}})$, and where we used contraction twice
to merge the $x$s and $y$s. Note that
$||(2\sqrt {2}, \sqrt {2})||_2=\sqrt {8+2}=\sqrt {10}$, which is why the final
sensitivities have this form.

By contrast, consider how we might attempt to type this program directly in the
original Fuzz. Let us assume that we are working in an extension of Fuzz with
types for expressing the domains of $f$ and $g$, similarly to the $L^2$ vector
types of Duet~\cite{DBLP:journals/pacmpl/NearDASGWSZSSS19}.  Moreover, let us
assume that we have coercion functions that allow us to cast from
$(!_2\R) \otimes_2 (!_2\R)$ to $(!_2\R) \otimes_2 \R$ and
$\R \otimes_2 (!_2 \R)$.  If we have a pair
$p : !_2 ((!_2 \R) \otimes_2 (!_2\R))$, we can split its sensitivity to call $f$
and $g$ and then combine their results with addition.  However, this type is
equivalent to $!_4 (\R \otimes_2 \R)$, which means that the program was given a
worse sensitivity (since $\sqrt {10}< 4$).

Of course, it would also have been possible to extend Fuzz with a series of
primitives that implement precisely the management of sensitivities performed by
bunches.  The point is that here this low-level reasoning is handled directly by
the type system.

\aaa{This last point is a bit weak, since we do not have an implementation of
  the type checker.}

\paragraph{Distributivity properties}

In linear logic the following distributivity properties are derivable:
\begin{align*}
  A \otimes (B \oplus C)  & \vdash (A \otimes B) \oplus (A \otimes C) \\
  (A \otimes B) \oplus (A \otimes C)  & \vdash A \otimes (B \oplus C) \\
  (A \with B) \oplus (A \with C) & \vdash A \with (B \oplus C).
\end{align*}
However, $\with$ does not distribute perfectly over $\oplus$, since the converse of
the last statement does not usually hold:
\begin{align*}
  A \with (B \oplus C)   \not\vdash (A \with B) \oplus (A \with C).
\end{align*}

By contrast, in \system{}, $\otimes_p$ does distribute over $\oplus$, as
witnessed by the following judgments
% , so this is particular the case for
%  $\otimes_1$ (corresponding to $\otimes$) and for   $\otimes_{\infty}$ (corresponding to $\with$). The corresponding terms are the following ones (for any $p$):
% With environment $\Gamma = [u : A \otimes_P (B \oplus C)]_1$ we can derive
% $\Gamma \vdash t : (A \otimes_p B) \oplus (A \otimes_p C)$ where $t$ is the
% program
\begin{align*}
[u : A \otimes_P (B \oplus C)]_1 & \vdash t_1 : (A \otimes_p B) \oplus (A \otimes_p C)\\
[u : (A \otimes_p B) \oplus (A \otimes_p C)]_1 & \vdash t_2 : A \otimes_p (B \oplus C),
\end{align*}
where
\begin{align*}
  t_1 = \LetPairIn {&u_1} {u_2} {u} {} \text{case } u_2 \text{ of}\\
    &|\;x.\;\inj_1(u_1,x)\\
    &|\;y.\;\inj_2(u_1,y)\\
  t_2 = \textbf{case }& u \textbf{ of}\\
    &|\; x.\;\LetPairIn{x_1}{x_1}{x}{(x_1, \inj_1 x_2)}\\
    &|\; y.\;\LetPairIn{y_1}{y_1}{y}{(y_1, \inj_2 y_2)}
\end{align*}

We can also show the following distributivity properties of scaling:
\begin{align*}
[x : A \otimes_p B]_r & \vdash t_1 : {!_r A} \otimes_p {!_r B}\\
[z : \!_r \!_sA]_1 & \vdash t_2 : \!_s \!_r A.
\end{align*}
where $t_1$ and $t_2$ are
\begin{align*}
  t_1 & = \LetPairIn {x_1} {x_2} {x} {(!_r x_1,\!_r x_2)}\\
  t_2 & = \LetBangIn{y}{z}{ \LetBangIn{w}{y}{!! w }  }.
\end{align*}

\paragraph{Programming with matrices}

The Duet language~\cite{DBLP:journals/pacmpl/NearDASGWSZSSS19} provides several
matrix types with the $L^1$, $L^2$, or $L^\infty$ metrics, along with primitive
functions for manipulating them.  In \system{}, these types can be defined
directly as follows
\[ \mathbb{M}_p[m,n] = \otimes_1^m \otimes_p^n \R. \] Following Duet, we use the
$L^1$ distance to combine the rows and the $L^p$ distance to combine the
columns.

One advantage of having types for matrices defined in terms of more basic
constructs is that we can program functions for manipulating them directly,
without resorting to separate primitives.  For example, we can define the
following terms in the language:
\begin{align*}
addrow &: \mathbb{M}_{p} [1,n] \otimes_1 \mathbb{M}_{p} [m,n]
\multimap \mathbb{M}_{p} [m+1,n]  \\
addcolumn &: \mathbb{M}_{1} [1,m] \otimes_1 \mathbb{M}_{1} [m,n]
\multimap \mathbb{M}_{1} [m,n+1] \\
addition &: \mathbb{M}_{1} [m,n] \otimes_1 \mathbb{M}_{1} [m,n] \multimap \mathbb{M}_{1} [m,n].
\end{align*}
The first program, $addrow$, appends a vector, represented as a $1 \times n$
matrix, to the first row of a $m\times n$ matrix. The second program,
$addcolumn$, is similar, but appends the vector as a column rather than a row.
Because of that, it is restricted to $L^1$ matrices.
%
\aaa{Can we generalize addcolumn to $L^p$ matrices? It feels like it should be
  possible, at least if we use $\otimes_p$ to separate the two arguments.}
%
Finally, the last program, $addition$, adds the elements of two matrices
pointwise.

One drawback of our encoding is that these programs need to be defined
separately for each matrix dimension.  In practice, it would be desirable to
have a dependently typed version of \system{}, along the lines of
DFuzz~\cite{DBLP:conf/popl/GaboardiHHNP13}, to simplify the manipulation of
matrices of arbitrary size.

\paragraph{Metrics for lists}

In Fuzz, we can define two list types using
recursion~\cite{DBLP:conf/icfp/ReedP10}:
\begin{align*}
\mathtt{list} \; A & = \mu \alpha. 1 \oplus (A \otimes \alpha) &
\mathtt{alist} \; A & = \mu \alpha. 1 \oplus (A \with \alpha).
\end{align*}
Let us denote as $L(A)$ the set of lists over $A$, which will be ranged over by
$l$.  Following prior work~\cite{DBLP:conf/popl/AmorimGHKC17}, these types can
be interpreted as metric spaces, by computing the initial algebra of a certain
functor.  This leads to the following metrics:
\begin{align*}
  d_{list}(l,l') & =
  \begin{cases}
    \infty & \text{if $|l| \neq |l'|$} \\
    \sum_{i=1}^{n} d_A(l_i,l'_i) & \text{if $|l| = |l'| = n$}
  \end{cases} &
  d_{alist}(l,l') & =
  \begin{cases}
    \infty & \text{if $|l| \neq |l'|$} \\
    \max_{i=1}^{n} d_A(l_i,l'_i) & \text{if $|l| = |l'| = n$}.
  \end{cases}
\end{align*}
Let us assume for the moment that we extend \system{} with inductive types, by
which we mean recursive types with strictly positive recursive occurrences.  We
can extend these definitions to arbitrary $L^p$ distances:
\[p\mathtt{list} \; A = \mu \alpha. 1 \oplus (A \otimes_p \alpha).\]  The category
of metric spaces has colimits of chains, so it should be possible to interpret
such recursive types as a colimit by arguing that strictly positive type
expressions correspond to cocontinuous functors on this category.  Unfolding
definitions, we obtain the following distance on this type:
\begin{align*}
  d_{plist}(l,l') & =
  \begin{cases}
    \infty & \text{if $|l| \neq |l'|$} \\
    \sqrt[p]{\sum_{i=1}^{n} d_A(l_i,l'_i)} & \text{if $|l| = |l'| = n$}.
  \end{cases}
\end{align*}
In the cases $p \in \{1,\infty\}$, this reduces to the previous distances on
lists (where, in the case $p = \infty$, we take the limit of the right-hand side
when $p \to \infty$).

The $\plist$ type is equipped with the following constructors:
\begin{align*}
nil &: \plist A \\
cons &:  A \otimes_p \plist A \multimap \plist A.
\end{align*}
Moreover, we can define functions on lists by structural recursion, assuming
that such a principle is provided as a combinator in \system{}.  For example:
\begin{align*}
  append &: \plist A  \otimes_p \plist A \multimap \plist A.
\end{align*}

\paragraph{Vector addition over sets}
Let us now show an example of a Fuzz term for which using $L^p$ metrics and
typing in \system{} allows to obtain a finer sensitivity analysis.

We consider sets of vectors in $\R^d$ and the function $\mathit{vectorSum}$
which, given such a set, returns the vectorial sum of its elements.  In Fuzz,
this function can be defined via a summation primitive
\[\mathit{sum} : {!_\infty (!_\infty A \multimap \R)} \multimap \Set A \multimap \R,\]
which adds up the results of applying a function to each element of a
set~\cite{DBLP:conf/icfp/ReedP10}.  The definition is as follows:
\begin{align*}
  \mathit{vectorSum} & : {!_d \Set(\otimes_1^d \R)} \multimap_1 \otimes_1^d \R \\
  \mathit{vectorSum}\;s & = (\mathit{sum}\;\pi_1\;s,\ldots,\mathit{sum}\;\pi_d\;s).
\end{align*}
Here, $\pi_i : \otimes_1^d \R \multimap \R$ denotes the $i$-th projection, which
can be defined by destructing a product.  Set types in Fuzz are equipped with
the Hamming metric \cite{DBLP:conf/icfp/ReedP10}, where the distance between two
sets is the number of elements by which they differ.  Note that, to ensure that
$\mathit{sum}$ has bounded sensitivity, we need to clip the results of its
function argument to the interval $[-1,1]$.  Fuzz infers a sensitivity of $d$
for this function because its argument is used with sensitivity 1 in each one of
the components of the tuple.

In \system{}, we can define the same function as above, but we also have the
option of using a different $L^p$ distance to define
$\mathit{vectorSum}$, which leads to the type
$!_{d^{1/p}} \Set(\otimes_p^d \R) \multimap \otimes_p^d \R$, with a sensitivity
of $d^{1/p}$.

For the sake of readability, we'll show how this term is typed in the case
$d=2$.  By typing each term  $(sum \; \pi_i \;z_i)$ and applying
$(\otimes I)$ we get:
$$  [z_1: \Set (\R \otimes_p \R) ]_1 \; ,_p  [z_2: \Set (\R \otimes_p \R)
]_1\vdash (sum \; \pi_1 \;z_1,sum \; \pi_2 \;z_2): \R \otimes_p \R. $$ By
applying the contraction rule, we obtain:
$$  [z : \Set (\R \otimes_p \R) ]_{2^{1/p}}  \vdash (sum \; \pi_1
\;z,sum \; \pi_2 \;z): \R \otimes_p \R. $$ The claimed type is finally obtained
by $(! E)$ and $(\multimap I)$.

\paragraph{Calibrating noise to $L^p$\/distance}
Hardt and Talwar~\cite{HardtT10} have proposed a generalization of the Laplace
mechanism, called the $K$-norm mechanism, to create a differentially private
variant of a database query $f:{\tt dB}\to \mathbb{R}^d$.  The difference is
that the amount of noise added is calibrated to the sensitivity of $f$ measured
with the $K$ norm, as opposed to the $L^1$ distance used in the original Laplace
mechanism.  When $K$ corresponds to the $L^p$ norm, we will call this the
$L^p$-mechanism, following Arwan and Slavkovich~\cite{osti_10183971}.

\begin{definition}
  Given $f:{\tt dB}\to \mathbb{R}^d$ with $L^p$ sensitivity $s$ and
  $\epsilon>0$, the $L^p$-mechanism is a mechanism that, given a database
  $D\in{\tt dB}$, returns a probability distribution over $y\in \mathbb{R}^d$
  with density given by:
\[
\frac{\exp(\frac{-\epsilon||f(D)-y||_p}{2s})}
{\int \exp(\frac{-\epsilon||f(D)-y||_p}{2s})d y}
\]
\end{definition}
This mechanism returns with high probability (which depends on the privacy
budget $\epsilon$ and on the sensitivity $s$ of $f$) a vector $y\in\mathbb{R}^d$
which is close to $f(D)$ in $L^p$ distance.  Such a mechanism can be easily
integrated in \system{} through a primitive:
$$
{\tt LpMech} :  {!_{\infty}(!_s {\tt dB}\multimap \otimes_p^d\mathbb{R})} \multimap {!_\epsilon {\tt dB}} \multimap  \bigcirc_P (\otimes^d_p\mathbb{R})
$$
(Strictly speaking, we would need some discretized version of the above
distribution to incorporate the mechanism in \system{}, but we'll ignore this
issue in what follows for simplicity.)

The fact that the ${\tt LpMech}$ satisfies $\epsilon$-differential privacy
follows from the fact that this mechanism can actually be seen as an instance of
the \emph{exponential mechanism}~\cite{McSherryT07}, a general tool to guarantee
differential privacy. This mechanism is based on a scoring function assigning a
score to every pair consisting of a database and a potential output, and it
attempts to return an output with approximately maximal score, given the input
database. As shown by Gaboardi et al.~\cite{DBLP:conf/popl/GaboardiHHNP13}, the
exponential mechanism can be added as a primitive to Fuzz with type:
$$
{\tt expmech} : {!_\infty \Set(\mathcal{O})} \multimap {!_\infty (!_\infty
  \mathcal{O} \multimap !_s {\tt dB}\multimap \mathbb{R})} \multimap
!_\epsilon{\tt dB} \multimap \bigcirc_P \mathcal{O},
$$
where $\mathcal{O}$ is the type of potential outputs.  The function
${\tt LpMech}$ is just an instance of the exponential mechanism where we take
$\mathcal{O}$ to be $\otimes^d\mathbb{R}$ and the scoring function to be
$\lambda y. \lambda D. ||f(D) - y||_p$.

To define the $L^p$ mechanism following this recipe, we would need to reason
about the sensitivity of this scoring function.  In Fuzz, this would not be
possible, since the language does not provide support for reasoning about the
sensitivity of $f$ measured in the $L^p$ distance.  In \system{}, on the other
hand, this can be done with no trouble. %Below, we will see two examples of how
%the $L^p$ mechanism can lead to more accurate privacy guarantees.
Below, we will see an example (Gradient descent) of how
the $L^p$ mechanism can lead to a more accurate privacy guarantee.
\pb{Modified this last sentence as finally we are not using the $L^p$
  mechanism for k-means but only for gradient descent.}

\paragraph{K-Means} The k-means algorithm is an iterative algorithm for
finding multiple means in a set of datapoints. These means can be
thought of as approximate "centers" of groupings in the dataset. A
differentially private version of the k-means algorithm typed in Fuzz had been given in \cite{DBLP:conf/icfp/ReedP10}, using the Laplace mechanism.
Here we revisit this example to
illustrate how by using \system{}  typing and $L^p$  one can refine the
sensitivity analysis of an algorithm.

 The $iterate$ Fuzz term defined in \cite{DBLP:conf/icfp/ReedP10}
 takes a set of data points, a list of centers and returns an updated
 list of centers, obtained by grouping each data point to the center
 it is closest to, adding Laplacian noise and then taking the new
 centers to be the mean of each group. It was given the following Fuzz
type\footnote{Actually there were two typos on types in
  \cite{DBLP:conf/icfp/ReedP10}; the type of $iterate$ given here is
the right corrected one, as well as the type of $zip$.}
$$ iterate : \!_{3} (\set pt) \multimap  \Fuzzlist pt \multimap    \bigcirc_P ( \Fuzzlist pt)$$
The 3 sensitivity of $iterate$ in its first data points set
  argument comes from the fact that this argument is used 3 times in
  the term, thus the Fuzz contraction rule (in $L^1$) leads to an
  index 3 for the $!$ of this argument. The  idea here is to use instead in
  \system{}  contraction in a $L^p$ bunch context, which will lead to
  an index $\sqrt[p]3$ instead of 3. For enabling that one needs to
  change the type of the $zip$ intermediate function, replacing
  $\multimap$ with $\multimap_p$. Then this forces to take for
  points  the type $pt=\R \otimes_p \R$ (so using the \lp metric), for lists the type $\plist A$,
  and to change accordingly the type of $map$ and of the other
  intermediary functions. We obtain the following types:

% \pb{I propose to remove the following sentences}
% \system{} allows us to define k-means for an arbitrary \lp space. We can see this affect the sensitivity of the program because the database is $\sqrt[p]3$ sensitive rather than in Fuzz where it is 3 sensitive. This is because Fuzz is written with the underlying metric space of $L^1$.

% % \jw{define pt as $\R \otimes_p \R$}

% % \jw{talk about how it's natural to write programs with arbitrary p norm in bunched fuzz}

% % \jw{point out sensitivity $\sqrt[p]{3}$ which is a small improvement here but indicative of how p norms affect sensitivity in other programs}

% % \jw{ensure that there are closed derivations of assign partition totx toty zip, and use these via weakening to prevent having having to manage these in the context}

% % \jw{make sure we can write the set helper functions using the primitives in bfuzz so we know the primitives are sound in bfuzz. watch out for L1 vs Lp}

% % \jw{can we prove that $A \otimes_p !_\infty B \text{ ISOMORPHIC TO } A \otimes_q !_\infty B$ ?}

% For k-means in \system{} we use the following helper functions:
% \pb{end of removed part}
\begin{align*}
  pt & \triangleq \R \otimes_p \R\\
  assign &: \plist pt \multimap_\infty \set pt \multimap_p \set (pt \otimes_p int)
  \\partition &: \set (pt \otimes_p int) \multimap_p \plist (\set pt)
  \\totx, toty &: \set pt \multimap \R
  \\zip &: \plist A \multimap_p \plist B \multimap_p \plist (A \otimes_p B)
  \\pmap &: \!_\infty(A \multimap_p B) \multimap_p (\plist A) \multimap_p plist B
\end{align*}

%We define the $pt$ type (read "point") to be a point in 2D space using
%the \lp metric for some arbitrary fixed $p$.
The term $assign$ takes a list of means and a database and returns pairs of points matched with the index of the closest mean given in the list of means. $partition$ takes these labeled points and splits them into a list of sets of points. $totx$ and $toty$ calculate the total of the x or y coordinates respectively in a set of points. $zip$ is the usual zip function on lists, and $pmap$ is the usual map function adapted to our fixed \lp space. Finally, $seq$ binds over every element in a list to take a list of distributions and return a distribution over lists. %\jw{mention what monad we're using for this example}

\begin{align*}
  &seq : \plist (\bigcirc_P \alpha) \multimap_p \bigcirc_P (\plist \alpha)\\
  &seq\; [] = []\\
  &seq\; x :: xs =
  \mLet{y}{x}{
    \mLet{ys}{seq\; xs}{
      \return\; y :: ys}}
\end{align*}
The k-means algorithm is defined below. The user supplies a database and a set of $k$ initial means. The means are either initialized to random points within the dataset or are the output of a previous iteration of the algorithm. The datapoints are then grouped by distance to each mean using $assign$ and new means are calculated by taking the average of each groups $x$'s and $y$'s.
\begin{align*}
 iterate : \!_{\sqrt[p] 3} (&\set pt) \multimap_p \plist pt \multimap_p
  \bigcirc_P (\plist pt)\\
  iterate\; b\; ms =\;&\LetBangIn{b'}{b}{
    \\ &\LetIn{b''}{partition\; (assign\; ms\; b')}{
      \\ &\LetIn{tx}{pmap (add\_noise \circ totx)\; b''}{
        \\ &\LetIn{ty}{pmap (add\_noise \circ toty)\; b''}{
          \\ &\LetIn{t}{pmap (add\_noise \circ size)\; b''}{
            \\ &\LetIn{stats}{zip\; (zip\; (tx, ty), t)}{
              \\ &seq\; (pmap\; avg\; stats)
            }
          }
        }
      }
    }
  }
\end{align*}

Note that if we take $p=1$ we have exactly the same type derivation as
in \cite{DBLP:conf/icfp/ReedP10} in Fuzz.

It is also possible to write a variant of this program which instead
of building two lists, one for component $x$ and one for component
$y$, builds a single lists of vectors  in $\R \otimes_p \R$ by using
a map on the function $\mathit{vectorSum}$ defined before. The sensitivity
obtained with respect to the set of data points argument  is then $1+2^{1/p}$. For this variant one only uses Bunched Fuzz
connective  $\otimes_p$ for the underlying vector type $\R \otimes_p
\R$ but one keeps the Fuzz versions (with $\multimap$) of $map$, $zip$, $assign$\dots
The noise is also added by the Laplace mechanism.

% Now let us present the second version of k-means. Here what we want to
% do is to compute directly on $\R \otimes_p \R$ vectors (points) and at
% the end add noise to $\R \otimes_p \R$ by using the   ${\tt LpMech}$
% mechanism. For that we consider a function $vectoradd$ which, given as
% argument a set of $\R \otimes_p \R$ vectors, returns the vector
% obtained by summing on each component. It can be defined from $tox$,
% $toty$ by:
% $$vectoradd= \lambda m. ((totx \; m) \otimes_p (toty \; m)): !_{
%   2^1/p}  \set pt \multimap pt$$
% Then the new function $iterate'$ is defined from $iterate$ by changing
% lines 3 to 6 by:
% \begin{align*}
% &\LetIn{tx}{pmap (add\_noise \circ totx)\; b''}\\
% &\LetIn{ty}{pmap (add\_noise \circ toty)\; b''}\\
% &\LetIn{t}{pmap (add\_noise \circ size)\; b''}\\
% &\LetIn{stats}{zip\; (zip\; (tx, ty), t)}

% \end{align*}

\paragraph{Gradient descent} Let us now give an example where we use
the $Lp$-mechanism. An example of differentially private gradient descent example
with linear model in Fuzz was given in
\cite{DBLP:journals/pacmpl/Winograd-CortHR17} (see Sect. 4.1, 4.2 and
Fig. 6 p. 16, Fig. 8 p.19). As k-means this is an iterable algorithm. Actually it was given for an extended language called
Adaptative Fuzz, but the code already gives an algorithm in (plain)
Fuzz. We refer the reader to this reference for the description of all
functions, and here we will only describe how one can adapt the
algorithm to \system{}.

Given a set of $n$ records $x_i \in \R^d$, each with a \textit{label}
$y_i \in \R$, the goal is to find a parameter vector $\theta \in \R^d$
that minimizes the difference between the labels and their
\textit{estimates}, where the estimate of a label $y_i$ is the inner
product $<x_i,\theta>$. That is, the goal is to minimize the loss
function defined as:
$$ L(\theta ,(x,y))= \frac{1}{n}\cdot
\Sigma_{i=1}^{n}(<x_i,\theta>-y_i)^2$$
The algorithm starts with an initial parameter vector $(0,\dots,0)$ and
it iteratively produces successive $\theta$ vectors until a
termination condition is reached.

  The Fuzz program uses the data-type $bag \; A$ representing bags or
  multisets over $A$. A $bagmap$ primitive is given for it. The type
  $I$ is the unit interval $[0,1]$.

 The main  function is called
$updateParameter$ and updates one component of the model $\theta$; it is computed
in the following way:
\begin{itemize}
\item with the function $calcGrad$ from ${\tt dB}$ to $\R$ compute one
  component  $(\nabla L( \theta,(x,y)))_j$ of the $\R^d$ vector
  $\nabla L( \theta,(x,y))$ \footnote{Actually $calcGrad$ computes
    $(\nabla L( \theta,(x,y)))_j$ up to a multiplicative constant,
    2/n, which is mutliplied afterwards in the $updateParameter$
    function. }.
\item  then a Laplacian noise is postcomposed with $calcGrad$ in the
  $updateParameter$ function. This uses a privacy budget of
  $2\epsilon$. It has to be done for each one of the
  $d$ components of $\nabla L( \theta,(x,y))$, thus on the whole, for
  one step, a
  privacy budget of  $2d\epsilon$.
\item The iterative procedure of gradient descent is given by the
  function $gradient$ in Fig. 8 p. 19 of
  \cite{DBLP:journals/pacmpl/Winograd-CortHR17}. We forget here about the
  adaptative aspect and just consider iteration with a given number
  $n$ of steps. In this case by applying $n$ times $updateParameter$
  one gets a privacy budget of $2d n\epsilon$.
 \end{itemize}
  We modify the program in the following ways in order to type it in
  \system{} and use the $L^p$-mechanism.

 Instead of computing over  $\R$ we want to compute over
 $ \otimes_p^d \R$ for a given $p\geq 1$, so $\R^d$ equiped with \lp
 distance. The records $x_i$ are in $ \otimes_p^d I$ and the labels
 $y_i$ in $I$. The database type is $dB=bag \; (I
 \otimes_p(\otimes_p^d I)) $. The distance between two bags in ${\tt dB}$
 is the number of elements by which they differ.

 We assume given a primitive $ bagVectorSum$ with type
 $!_{d^{1/p}} bag \; ( \otimes_p^d I) \multimap \otimes_p^d \R$ (it could be
 defined as the $\mathit{vectorSum}$ defined above for sets, using a $sum$
 primitive for bags). Given a bag $m$, $(bagVectorSum \; m)$ returns the
 vectorial sum of all elements of $m$. One can check that the sensitivity of
 $ bagVectorSum$ is indeed $d^{1/p}$ because given two bags $m$ and $m'$ that
 are at distance 1, if we denote by $u$ the vector by which they differ, we
 have:
\begin{align*}
d_{(\otimes_p^d \R) }(bagVectorSum (m),bagVectorSum (m'))   &= ||u
||_p = (\Sigma_{j=1}^d |u_j|^p)^{1/p}  \\
  & \leq  (\Sigma_{j=1}^d 1)^{1/p}  = d^{1/p}
\end{align*}
By adapting the $calcGrad$ Fuzz term of
\cite{DBLP:journals/pacmpl/Winograd-CortHR17} using $ bagVectorSum$ we obtain a
term $VectcalcGrad$ with the following \system{} type:
$$ VectcalcGrad: !_{\infty} \otimes_p^d \R \multimap !_{d^{1/p}} dB
\multimap  \otimes_p^d \R$$
Given a vector $\theta$ and a database $(y,x)$,  $ VectcalcGrad$
computes the updated vector $\theta'$. Finally we define the term
$updateVector$ by adding noise to $ VectcalcGrad$ using the the
$L^p$-mechanism. Recall that the type of ${\tt LpMech}$ is:
% $$
% {\tt LpMech} : (!_s {\tt dB}\multimap \otimes_p^d\mathbb{R})\multimap !_\epsilon {\tt dB} \multimap  D (\otimes^d_p\mathbb{R})
% $$
$$
{\tt LpMech} :  !_{\infty}(!_s {\tt dB}\multimap \otimes_p^d\mathbb{R})\multimap !_\epsilon {\tt dB} \multimap  \bigcirc_P (\otimes^d_p\mathbb{R})
$$
We define $ updateVector$ and obtain its type as follows:
$$ updateVector= \lambda \theta. ({\tt LpMech} \; (VectcalcGrad \;
\theta)):  \; !_{\infty} \otimes_p^d \R \multimap !_\epsilon {\tt dB}
\multimap  \bigcirc_P ( \otimes_p^d\R) $$
By iterating $ updateVector$ $n$ times one obtains a privacy budget of $n
\epsilon$.

\pb{I am not quite sure about how the privacy budget of this Bunched
  Fuzz/LpMech version compares to the privacy budget of the original
  Fuzz/Laplace mech version. }




==> sect_motivational_introduction.tex <==
%\section{Motivational introduction to the logic:}

\begin{itemize}
\item Fuzz and linear logic:

 As explained in %\
cite{ReedPierce2010},
 one intuition behind the design of the Fuzz language is that  \textit{the capability to sensitively depend on an input's value behaves like a resource}.
 Hence as linear logic is a logical system handling formulas as resources, it has inspired the type system for Fuzz. The linear arrow of linear logic $\multimap$ corresponds in Fuzz to the type of a $1$-sensitive function. The $!$ (bang) modality is employed in linear logic to represent multiple uses of a formula/argument,  and the analog $!_r$ in Fuzz, indexed by a real number $r$, represents scaling of a types' metric by factor $r$: $d_{!_r \tau}(x,y)=r \cdot d_{!_r \tau}(x,y)$. Products and coproducts in Fuzz types respectively correspond to the $\&$ and $\oplus$ connectives of linear logic (additive conjunction and disjunction).

However the type system of Fuzz has some limitations.  A first observation is that programming linearly, that is to say by using arguments at most once, or -- equivalently -- without the $!$ modality in linear logic, imposes some restrictions. One example given in  %\
cite{ReedPierce2010} (Sect 3.3) 
 is when a function taking as input a pair wants to case analyze one component of that pair without consuming the other component. This can be achieved with a function  \textit{analyze} with the following type: $A \& (B \oplus C)  \multimap (A \& B) \oplus (A \& C)$. This formula represents a distributivity property and is \textit{not}  provable in linear logic, hence  \textit{analyze}  cannot be programmed in this system and has to be added as a primitive.

 A second observation is that Fuzz types allow to define $\ell^1$ (with the $\otimes$ connective) and  $\ell^\infty$ (with $\&$) metrics, which are specific cases of the  $\ell^p$  family of metrics, for $p\geq 1$. For instance   the $\ell^2$ metric is used by the Gaussian mechanism in differential privacy, but cannot be managed by Fuzz types. One of our goals is thus to extend the type system in order to account for arbitrary $\ell^p$  metrics, for $p\geq 1$. A natural idea for that is to consider a family of connectives $\otimes_p$ indexed by $p$. However this requires to also generalize sequents (or typing environments, if one takes the typing point of view) by  replacing the unique  \textit{comma}  constructor on sequents $\Gamma, \Delta$ by  $\Gamma,_p \Delta$ where \textit{comma}  is indexed by $p$.

 Interestingly enough these two remarks suggest to move to another logical setting, that of bunched logic cite{DBLP:journals/bsl/OHearnP99}.  First, as pointed in \
cite{ReedPierce2010} (Sect 3.3) footnote 2, the logic of bunched implications BI, contrarily to linear logic,  satisfies the distributivity property $A \& (B \oplus C)  \multimap (A \& B) \oplus (A \& C)$. Second, introducing several  \textit{comma}  $,_p$ constructors on sequents leads to the definition of bunches.

%\item generalizing the product, and relationship to bunched logic

 \item how to deal with other measures on probabilities, hellinger and how we captured it 
          in the lics paper (more on the calculus) :  TO BE DONE


\end{itemize}
